Arena-Lite: Efficient and Reliable Large Language Model Evaluation via Tournament-Based Direct Comparisons

As Large Language Models (LLMs) expand across domains, LLM judges have become essential for systems evaluation. Current benchmarks typically compare system outputs against baselines. This baseline-mediated approach, though convenient, yields lower reliability than direct comparison between systems. We propose Arena-Lite which integrates tournament structure on top of head-to-head comparison. The application of a tournament structure and direct comparison eliminates the need for baseline outputs, reduces the number of required comparisons, and allows higher reliability in system rankings. We conducted two experiments: (1) controlled stochastic modeling and (2) empirical validation with a real LLM judge. Those experiments collectively demonstrate that Arena-Lite consistently achieves higher reliability with fewer comparisons, even with smaller datasets or weaker judges. We release an easy-to-use web demonstration and code to foster adoption of Arena-Lite, streamlining model selection across research and industry communities. Arena-Lite demo and code are available on \href{https://huggingface.co/spaces/NCSOFT/ArenaLite}{https://huggingface.co/spaces/NCSOFT/ArenaLite}

==> DEPRECATE/4_experimental_settings.tex <==
\section{Experimental Settings}
 We run modeling experiment for testing our foundational proposition for \textit{\textbf{Varco Arena}} design mentioned in section~\ref{sec:Tournaments of LLMs over multiple prompts} that performing tournaments over the prompts in benchmark helps sorting the models in their skills. By this simulation, we would find that the effectiveness of the tournament approach is valid for ranking LLMs without the intervention of unnecessary factors such as biases in LLM judges~\cite{Offsetbias}. And with the following empirical experiments with Judge LLM, we clearly compares our approach on LLM benchmarking against the current practice; tournament vs. comparing to reference as an \textit{anchor} comparison. Note that reference as an \textit{anchor} or \textit{anchored comparison} approach indicates the current approach of using reference as a comparison baseline to benchmark LLMs. Before that, we describe why we put leaderboard rankings from Chatbot Arena as a ground truth to measure those approaches over. 

\subsection{Ratings from Chatbot Arena Leaderboard as a Ground-Truth LLM Rankings}\label{sec:Ratings from Chatbot Arena Leaderboard as a Ground-Truth LLM Rankings}
 We take the rankings from the Chatbot Arena leaderboard, and compare the result of each benchmarking approach against it. So far, Chatbot Arena is considered one of the most reliable leaderboard in terms of the number of human preference annotations. Chatbot Arena asks a user to decide which response from a pair of  LLMs is preferable, based on a user's attempt to prompt the models with a same query. Considering the vast number of votes, and the extensive coverage of the submitted prompts for model comparison, the resultant ranks from Chatbot Arena is likely to be quite accurate enough to be deployed as a ground-truth rankings. Chatbot Arena provides categorized leaderboard according to the prompts used for computing the Elo ratings and ranks for leaderboard, we consider leaderboard rankings from the \textit{Hard prompts} category adds reliability of real indication of LLM capability. \textit{Hard prompt} category leaderboard used $<$30\% of the total user annotation submitted to the platform which is around 450K number of matches assorted by considering how helpful a match is for differentiating LLMs.
 
 
\subsection{Simulating Unbiased Judge}
\label{sec:Simulating Unbiased Judge}
 Based on the argument we presented in section~\ref{sec:Tournaments of LLMs over multiple prompts}, we designed simple stochastic model of an LLM matches with another. The foundational assumption we are making here is that In this model, the outcome of the match is determined with probability governed by a latent factor, Elo rating, and we do not distinguish the prompts in the benchmark dataset complying to the argument. All the other factors that may affect the match outcome is simplified into a factor, \textit{judge precision} which is represented as a likelihood of a judge to make a correct decision. To detail further, core variables for the simulation model are as follow: 
 \begin{enumerate}
 \item Elo ratings of the models: Outcome of a single match is determined by stochastic manner regarding the Elo gap between the models. The Elo ratings are extracted dating back to June 23, from English category of a Chatbot Arena.\footnote{Different from empirical experiment, ground-truth Elo ratings are from \textit{overall} category, not \textit{hard prompts}. This does not affect the validity of our simulation as it is equivalent to simulation run for different set of LLMs.}
 \item Judge Precision: We cram all the sophistication of a single match over a prompt to a stochastic modeling of a judge that has precision of deciding correct winner according to the Elo rating of a participants. 
 \end{enumerate}
Thus the likelihood of an \textit{correct} outcome (i.e. model of higher rate wins) single match is as follows in Equation~\ref{eq:correct_outcome_likelihood}. $P_\text{predict}$ is outcome likelihood, $P_\text{judge}$ is the precision of a judge, $P_\text{gt}$ is the expected win rate of $M_i$ over $M_j$ as in Equation~\ref{eq:bt_model_elo} and $\Delta_\text{ij}$ is rate gap between those ($R_i - R_j$). 
\begin{equation}
P_\text{predict}(i> j) = P_\text{judge} * P_\text{gt}(i> j) 
                         = P_\text{judge} * \frac{1}{1+10^{\Delta_\text{ij}/400}}
    \label{eq:correct_outcome_likelihood}
\end{equation}
 Actual process of the simulation goes as follows: (1) First, we choose participants from the top of the Chatbot Arena leaderboard with skipping models that tied (i.e. if we see two 4th place, we take only one of those), and (2) from the Elo ratings of the participants, we compute the expected win rate matrix, say $A$ where $a_\text{ij} = P_\text{gt}(i>j )$. (3) Unbiased judge of $P_\text{judge}$ will behave according to Equation~\ref{eq:correct_outcome_likelihood} regarding only Elo gap $\Delta_\text{ij}$ for any attempted match.\footnote{Iterating over various test prompts in benchmark is simplified as repeating to sample judge outcome from the Equation~\ref{eq:correct_outcome_likelihood} In practice, difficulty of the prompt will affect the quality of the LLM output, as well as judge precision, but we assume we are perfectly controlling it}. (4) Sample required set of matches to start the tournaments or \textit{anchored comparisons} over the test prompts. This degenerates to sampling wanted number of match outcomes for designated pair of models as we regard all the prompts as indistinguishable. (5) All the match outcomes sampled are recorded with winner and the match-up. And then, (6) we figure out the scores for ranking. For \textit{anchored comparison approach}, the score is win rate to reference LLM, that is win rate against the \texttt{gpt-4-1106-preview} (Elo rate of 1233), and for tournament, estimated Elo ratings from the recorded match outcomes. (7) Obtained ranks from (6) is compared with original rank from the ground truth Elo rate where we started our simulation. To alleviate randomness from the tournament bracket and sampling output results, we performed 50 trials per any configuration.
 
  By simulation, we controlled three conditions for testing robustness and reliability of the two benchmarking approaches. We controlled the number of the participant models ($n_\text{models}$), number of benchmark size ($|X|$), and the judge precision ($P_\text{judge}$). 
 
\subsection{Running \textit{Varco Arena} with LLM-as-a-Judge}
 To practical validation of our propositions, we compare the two approaches with controlled conditions for two scenarios of running \textit{\textbf{Varco Arena}} as mentioned in section~\ref{sec:Possible Usage Scenarios of LLM Benchmarks with Varco Arena}. As a list of models to be ranked, we choose 21 LLMs' from the top of ChatBot Arena (\textit{hard prompts}) leaderboard, and use Arena-Hard-Auto prompts and their reserved outputs for our experiment. Note that excluding judge and anchor model are excluded from participants to avoid egocentric bias \cite{egocentric} makes the leaderboard listed with 19 or 20 models, not 21. We use \texttt{gpt-4o-2024-05-13} as our judge, \texttt{gpt-4-0314} as an reference (anchor) model to perform \textit{anchored comparisons on}. LLM judge is prompted with pairwise comparison referring to~\cite{LLMBar}, equally for both approaches. We also alternate the position of the model outputs to avoid positional bias. Details for LLM-as-a-judge configuration is further detailed on Appendix~\ref{appendix:Prompts and Judge configuration}. While \texttt{gpt-4o-2024-05-13} as a judge is quite realistic setting for LLM benchmarking, we also explore the use of \texttt{gpt-4o-mini-2024-07-18} as a judge considering budget tight situation. To assure statistically significant number of trials for each approach, but within the budget, we use Batch API serviced by OpenAI to prepare full-grid match outcomes as a cache file and reuse the match outcomes from the cache.

\subsection{Metrics and Bootstrapping}
 For measuring reliability of resulting rank of LLMs, we compute Spearman correlation coefficient between the rankings result computed by each approach run with Arena-Hard data, and the ground-truth leaderboard (i.e. rankings from Chatbot Arena). The Spearman coefficient ranges from 1 to -1 which interprets to perfect monotonic increment and decrement respectively (i.e. 1 interprets to copying the rankings in ground truth leaderboard).
 % We also provide bootstrapped results of the original observation to assure the robustness of the results presented. For empirical \textit{\textbf{Varco Arena}} experiment, we queried all-play-all matches, and using those, sampled 500 trials per configuration to ensure the reliable result under randomness. Otherwise specified, we stick to the median statistics for bootstrapping since the actual outcome rank to be seen is the result of single run, not the aggregation of massive number of repetition. 


==> DEPRECATE/5_results.tex <==
\section{Results}
We report the reliability of \textit{\textbf{Varco Arena}} for ranking multiple LLMs at once. In both simulated and empirical results, \textit{tournament approach} that \textit{\textbf{Varco Arena}} takes results in more aligned ranks to ground-truth Elo ranks. 

\subsection{Unbiased Judge Simulation}
\begin{figure*}

    \includegraphics[width=\textwidth]{APPENDIX_FIG/simul/merged_main_horizon.png}
    \caption{Simulated results of \textit{tournament} and \textit{anchored comparison} approach with unbiased judge. Gap between \textit{tournament} and \textit{anchored comparison} approach remains robust over varying numbers of participant LLMs ($n_\text{models}$), number of prompts in benchmark set ($|X|$) or judge precision ($P_\text{judge}$)}.
    \label{fig:anchored_vs_tournament_judge_precision_simulation}    
\end{figure*}
A set of whisker plots in Figure ~\ref{fig:anchored_vs_tournament_judge_precision_simulation} shows that the tournament approach appears to be more reliable evidenced by clear gaps in Spearman correlation. We tested if the gaps remain remarkable under varied configurations; Number of participant LLMs ($n_\text{models}$), prompts in benchmark set ($|X|$), and judge precision ($P_\text{judge}$)). We observe that the gaps remain clear between the tournament and \textit{anchored} approach regardless of how challenging the benchmarking condition becomes. While our simulation seems to run over an oversimplified model run by `judge precision ($P_\text{judge}$)' and the assumption of bias-free judge, we found that our simulation hints at the empirical results quite nicely. 

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{APPENDIX_FIG/empirical/empirical_merged.png}
    \caption{\textit{Tournament} and \textit{anchored comparison} shows a diminished correlation gap in empirical results, however, the overall trend from simulation experiments remains still. The gap between the two approaches reveals more clearly for running with weaker judges. \texttt{gpt-4o} as a judge shows the reduced gap between approaches while the gaps are clearer for \texttt{gpt-4o-mini} (right). Summarized numbers are represented in Table \ref{table:anchored_vs_tournament_n_prompts}}
        \label{fig:anchored_vs_tournament_n_prompts_gpt4o}

\end{figure}


\begin{figure*}
    \centering
    \includegraphics[width=1\textwidth]{figures/bar_with_ci_vs_chatbot_arena_gpt4o_500arenahard.png}
    \caption{Elo ratings of the model with gpt-4o judge on the full set of Arena-Hard-Auto~\cite{arena_hard} prompts. \textit{\textbf{Varco Arena}} result (bootstrapped median over 1000 samples of 500 results) is in blue, plotted alongside the ratings from Chatbot Arena (\textit{hard prompts}) in red. The median result is provided with a 95\% confidence interval, estimated using 1000 bootstrapped samples from 500 experiments, as done in the statistics notebook of~\cite{chatbot_arena}.}
    \label{fig:bar_with_ci_vs_chatbot_arena_gpt4o}
\end{figure*}




\subsection{Running \textit{Varco Arena} with \texttt{gpt-4o[-mini]} Judge}
 We could confirm that the same trend is being reproduced for empirical experiments, benchmarking LLMs with LLM-as-a-judge. As showcased in Figure~\ref{fig:anchored_vs_tournament_n_prompts_gpt4o} and Table~\ref{table:anchored_vs_tournament_n_prompts}, gaps become closer but slightly higher correlation for \textit{tournament} approach is observed across the varying benchmark size ($|X|$, denoted as $n_\text{prompts}$ in Figure~\ref{fig:anchored_vs_tournament_n_prompts_gpt4o}). 

\begin{table}[h]
\centering
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{lccccc}
    \hline
       Spearman corr. ($\uparrow$)& $|X|$ = 50& 100 & 250 & 475 & 500 \\
    \hline
    anchored (4o)  & 0.895 & 0.935 & \textbf{0.963} & 0.966 & 0.964 \\
    tournament (4o)  & \textbf{0.905} & \textbf{0.940} & 0.960 & \textbf{0.970} & \textbf{0.970} \\
    \hline
    anchored (4o-mini) & 0.895 & 0.908 & 0.917 & 0.916 & 0.912 \\
    tournament (4o-mini) & \textbf{0.901} & \textbf{0.919} & \textbf{0.931} & \textbf{0.933} & \textbf{0.933} \\
    \hline
    \end{tabular}
    }
    \caption{Spearman correlation ($\uparrow$) varying over size of the benchmark set ($|X|$) for each benchmarking approach. Median value from 500 trials. Details of the results are further represented by whisker plots in Figure \ref{fig:anchored_vs_tournament_n_prompts_gpt4o}}
\label{table:anchored_vs_tournament_n_prompts}
\end{table}

 
 While the gaps diminish for empirical results, it is notable that the \textit{tournament approach} does not require reference text as a comparison \textit{anchor}, and saves the number of comparisons for benchmarking ($|X| / n_\text{models}$ number of comparisons saved). According to the observation, gaps are clearer for changing weaker judges. Based on this, we could possibly project our expectation to the situation of using harder prompts. As the prompts get harder for the judge to make the correct decision (i.e. incurring lower judge precision), \textit{tournament} becomes more reliable compared to \textit{anchored comparison} approach. The visualized result is from sampled 500 experiments for each configuration (i.e. 500 stratified-random subsets of prompts sampled from the benchmark dataset for both \textit{tournament} and \textit{anchored} approach for $|X|$<500.\footnote{For $|X|$=500, using the full set of prompts from Arena-Hard-Auto, randomness only applies for \textit{\textbf{Varco Arena}} for its random initial match-up per prompt} For resultant Elo ratings compared with ground-truth from Chatbot Arena leaderboard, refer to Figure~\ref{fig:bar_with_ci_vs_chatbot_arena_gpt4o}.


